The Parallel Persistent Memory Model

We consider a parallel computational model that consists of $P$ processors, each with a fast local ephemeral memory of limited size, and sharing a large persistent memory. The model allows for each processor to fault with bounded probability, and possibly restart. On faulting all processor state and local ephemeral memory are lost, but the persistent memory remains. This model is motivated by upcoming non-volatile memories that are as fast as existing random access memory, are accessible at the granularity of cache lines, and have the capability of surviving power outages. It is further motivated by the observation that in large parallel systems, failure of processors and their caches is not unusual. Within the model we develop a framework for developing locality efficient parallel algorithms that are resilient to failures. There are several challenges, including the need to recover from failures, the desire to do this in an asynchronous setting (i.e., not blocking other processors when one fails), and the need for synchronization primitives that are robust to failures. We describe approaches to solve these challenges based on breaking computations into what we call capsules, which have certain properties, and developing a work-stealing scheduler that functions properly within the context of failures. The scheduler guarantees a time bound of $O(W/P_A + D(P/P_A) \lceil\log_{1/f} W\rceil)$ in expectation, where $W$ and $D$ are the work and depth of the computation (in the absence of failures), $P_A$ is the average number of processors available during the computation, and $f \le 1/2$ is the probability that a capsule fails. Within the model and using the proposed methods, we develop efficient algorithms for parallel sorting and other primitives.

==> preliminaries.tex <==
\section{Preliminaries}

Define the external memory model.

Define a RAM as we use it.   In particular it has $O(\log M)$ bits for a memory of size $M$, and has a set
of registers.

Define the A-RAM.

Define the asynchronous RAM.

Define lock-free and wait free.

Introduce work-stealing.

==> single-proc-proofs.tex <==
\section{Single Processor Proofs}\label{sec-single-proc-proofs}

This section provides the proofs of Theorem~\ref{theorem:RAM}
and~\ref{theorem:ideal-cache}.


\begin{proof} [Proof of Theorem~\ref{theorem:RAM}]
The simulation keeps all simulated memory in the \permem{} one word
per block.  It also keeps two copies of the registers in \permem{},
and the simulation swaps between the two.  At the end of a capsule on
one copy, it sets the restart pointer to a location just before the
other copy.  The code at that location, run at the start of the next
capsule, copies the other copy of the registers into the current copy,
and then simulates one instruction given by the program counter, by
reading from the other copy of the registers, and writing to the
current copy of registers (typically just a single register).  The
instruction might involve a read or write to the simulated memory, and
an update of the program counter either to the next simulated
instruction, or if a jump, to some other instruction.  Once the
instruction is done, the other copy of the registers is installed.
This repeats.  The capsules are read-write conflict free because they
only read from one set of registers and write to the other, and the
simulated memory instructions do a single read or write.  Every
simulated step takes a constant number of reads and writes to the
\permem{}.  Because the probability of a fault is constant the expected
number of repeats is constant.  The theorem follows.
%% We note that the simulation could simulate multiple steps within a
%% capsule, as long as it stops before a read-write conflict happens in
%% the simulated memory (i.e. the original RAM program reads and writes
%% the same location). \julian{Then capsule work is not necessarily $O(1)$?}
\end{proof}

\begin{proof} [Proof of Theorem~\ref{theorem:ideal-cache}]
  The simulation is similar to our external memory simulation,
  using rounds consisting of a \emph{simulation} capsule and a
  \emph{commit} capsule.  During each simulation capsule a simulated
  cache of size $2M/B$ blocks is maintained in the \locmem{}.  The
  capsule starts by loading the registers, and with an empty cache.
  During simulation, entries are never evicted, but instead the
  simulation stops when the cache runs out of space, i.e., after $2M/B$
  distinct blocks are accessed.  The capsule then writes out all dirty
  cache lines (together with the corresponding \permem{} address for
  each cache line) to a buffer in \permem{}, saves the registers and
  installs the commit capsule.  The commit capsule reads in the
  buffer, writes out all the dirty cache lines to their correct
  locations, and installs the next simulation capsule.  The simulation
  is read-write conflict free.

  We now consider the costs of the simulation.  $O(M)$ \locmem{} is
  sufficient to simulate the cache of size $2M$.  The total faultless work of a
  simulation capsule (run once) is bounded by $O(M/B)$ because we only
  have $2M/B$ misses before ending, and then have to write out at most
  $2M/B$ dirty cache blocks.  Accounting for faults, the total cost
  is still $O(M/B)$---given constant probability of faults.  The
  size of the cache and cost are similarly bounded for the commit
  capsule.  We now note that over the same simulated instructions, the
  ideal cache will suffer at least $M/B$ cache misses.  This is
  because the simulation round accesses $2M/B$ distinct locations, and
  only $M/B$ of them could have been in the ideal-cache at the start
  of the round, in the best case.  The other $M/B$ must therefore suffer
  a miss.  Therefore because each simulation round simulates what were
  at least $M/B$ misses in the ideal cache model with at most $O(M/B)$
  expected cost in the \ourmodel{} model, the theorem follows.
\end{proof}


==> ws-deque-code-ABP-style.tex <==
\begin{figure}\label{WS-deque-fig}
{\small

\begin{lstlisting}[language=C, numbers=left]
P = number of procs
S  = stack size

struct procState {

  union entry = empty
              | local
              | job of continuation
              | taken of (entry*,int)

  stack (int,entry)[S];
  int top;
  int bot;
  int ownerID;

  step(i) {
    return stack[i].first;
  }
  
  clearBottom() {
    stack[bot] = (step(bot)+1,empty);
  }

  helpPopTop() {
    t = top;
    switch(stack[top]) {
      case taken(ps,i):
        CAM(ps, (i,empty), (i+1,local)) // Set thief state.
        CAM(&top, t, t+1)    // Increment top.
        CAM(&bot, t, t+1)    // Increment bottom if local entry is stolen.
    }
  }

  // Steal from current processor, if possible.
  // If a steal happens, location e is set to "local"
  // and a job is returned. Otherwise NULL is returned.
  popTop(entry* e, int c) {
    helpPopTop();
    i = top;
    old = stack[i];
    commit;
    switch(old) {
      // No jobs to steal and no ongoing local work.
      case (j,empty): return NULL;
      // Someone else stole in meantime.  Help it.
      case (j,taken(_)): helpPopTop(); return NULL;
      // Job available, try to steal it with CAM.
      case (j,job(continuation)): 
        new = (j+1,taken(e,c));
        CAM(&stack[i], old, new);
        helpPopTop();
        if (stack[i] != new) return NULL;
        return continuation;
      // No jobs to steal, but there is local work.
      case (j,local): 
        // Try to steal local work if processor is dead.
        if dead[ownerID] {
          new = (j+1,taken(e,c))
          CAM(&stack[i], old, new);
          helpPopTop()
          if (stack[i] != new) return NULL;
          return activeCapsule[ownerID];
        }
        // Otherwise, return NULL.
        return NULL;
    }
  }

  pushBottom(continuation) {
    b = bot;
    t1 = step(b+1);
    t2 = step(b);
    commit;
    stack[b+1] = (step(b+1)+1,local);
    CAM(&stack[b], (t2,local), (t2+1,job(continuation));
    bot = b + 1;
    return;
  }

  popBottom() {
    b = bot;
    old = stack[b-1];
    commit;
    if (old == (j, job(continuation))) {
      CAM(&stack[b-1], old, (j+1,local));
      if (stack[b-1] == (j+1,local)) {
        bot = b-1;
        return continuation;
      }
    }
    // If we fail to grab a job, return NULL.
    return NULL;
  }

  schedule(set<continuation> jobs) {
    // Push all but one job onto the executor's WS-Deque.
    while(jobs.size > 1){
      states[getProcNum()].pushBottom(jobs.pop());
    }
    if (jobs.size == 1){
      children = execute(jobs[0]);
      GOTO(states[getProcNum()].schedule(children));
    } else {
      GOTO(states[getProcNum()].findWork();
    }
  }
  
  findWork() {
    clearBottom();
    newJob = popBottom();
    while (newJob == NULL){
      yield();
      victim = rand(P);
      i = step(bot);
      newJob = popTop(&stack[bot],i);
    }
    GOTO(states[getProcNum()].schedule(set<continuation>(newJob)));
  }
}
procState states[P];
\end{lstlisting}
}

\caption{Fault-tolerant WS-Deque Implementation}
\end{figure}


==> ws-deque-code.tex <==
\lstset{basicstyle=\footnotesize\ttfamily}
\lstset{escapeinside={@}{@}, literate={<}{{$\langle$}}1  {>}{{$\rangle$}}1}
\lstset{language=C, morekeywords={CAM,commit,empty,local,job,taken,entry,GOTO}}
\lstset{xleftmargin=5.0ex, numbers=left, numberblanklines=false, frame=single}

\begin{figure}
\begin{lstlisting}[firstnumber=1]
P = number of procs
S  = stack size

struct procState {
  union entry = empty
              | local
              | job of continuation
              | taken of <entry*,int>

  <int,entry> stack[S];
  int top;
  int bot;
  int ownerID;

  inline int getStep(i) { return stack[i].first; }
  
  inline void clearBottom() {
    stack[bot] = <getStep(bot)+1, empty>; }

  void helpPopTop() {
    int t = top;
    switch(stack[top]) {
      case <_, taken(ps,i)>:
        // Set thief state.
        CAM(ps, <i,empty>, <i+1,local>); @\label{line-help-set-local}@
        CAM(&top, t, t+1);    // Increment top.
   } }

  // Steal from current process, if possible.
  // If a steal happens, location e is set to "local"
  // & a job is returned. Otherwise NULL is returned.
  continuation popTop(entry* e, int c) {
    helpPopTop();
    int i = top;
    <int, entry> old = stack[i];
    commit;
    switch(old) {
      // No jobs to steal and no ongoing local work.
      case <j, empty>: return NULL;
      // Someone else stole in meantime.  Help it.
      case <j, taken(_)>: 
         helpPopTop(); return NULL;
      // Job available, try to steal it with a CAM.
      case <j, job(f)>: @\label{line-steal-job-case}@
        <int, entry> new = <j+1, taken(e,c)>;
        CAM(&stack[i], old, new); @\label{line-steal-job}@
        helpPopTop();
        if (stack[i] != new) return NULL;
        return f; @\label{line-poptop-return-job}@
      // No jobs to steal, but there is local work.
      case <j, local>: @\label{line-steal-local-case}@
        // Try to steal local work if process is dead.
        if (isDead(ownerID) && stack[i] == old) {
          <int, entry> new = <j+1,taken(e,c)>;
          stack[i+1] = <getStep(i+1)+1, empty>; @\label{line-avoid-extra-steal}@
          CAM(&stack[i], old, new); @\label{line-steal-local}@
          helpPopTop();
          if (stack[i] != new) return NULL;
          return getActiveCapsule(ownerID); @\label{line-poptop-return-local}@
        }
        // Otherwise, return NULL.
        return NULL;
  }  }

  void pushBottom(continuation f) {
    int b = bot;
    int t1 = getStep(b+1);
    int t2 = getStep(b);
    commit;
    if (stack[b] == <t2, local>) { @\label{line-pushBottom-if}@
      stack[b+1] = <t1+1, local>; @\label{line-pushBottom-new-local}@
      bot = b + 1; @\label{line-pushBottom-new-bot}@
      CAM(&stack[b], <t2, local>, <t2+1, job(f)> @\label{line-pushBottom-CAM}@
    } else if (stack[b+1].second == empty) {
      states[getProcNum()].pushBottom(f);
    }
    return;
  }

\end{lstlisting}
\end{figure}
\begin{figure}
\begin{lstlisting}[firstnumber=79]
  continuation popBottom() {
    int b = bot;
    <int, entry> old = stack[b-1];
    commit;
    if (old == <j, job(f)>) {
      CAM(&stack[b-1], old, <j+1,local>); @\label{line-popBottom-CAM}@
      if (stack[b-1] == <j+1, local>) { @\label{line-popBottom-check-CAM}@
        bot = b-1;
        return f;
      }   }
    // If we fail to grab a job, return NULL.
    return NULL;
  }

  ^ findWork() {
    // Try to take from local stack first.
    continuation f = popBottom();
    if (f) GOTO(f); @\label{line-bottom-pop-GOTO}@
    // If nothing locally, randomly steal.
    while (true) {
      yield();
      int victim = rand(P);
      int i = getStep(bot);
      continuation g 
          = states[victim].popTop(&stack[bot],i); @\label{line-call-popTop}@
      if (g) GOTO(g); @\label{line-top-pop-GOTO}@
    }
  }
}

procState states[P]; // Stack for each process.

// User call to fork.
void fork(continuation f) {@\label{line-fork}@
  // Pushes job onto the correct stack.
  states[getProcNum()].pushBottom(f);
}

// Return to scheduler when any job finishes.
^ scheduler() {@\label{line-scheduler}@
  // Mark the completion of local thread.
  states[getProcNum()].clearBottom();
  // Find work on the correct stack.
  GOTO(states[getProcNum()].findWork());
}
\end{lstlisting}

\caption{Fault-tolerant WS-Deque Implementation.
Jumps are marked as \texttt{GOTO} and
functions that are jumped to and do not return (technically
continuations) are marked with a \texttt{\^}.
%\phil{figure out a way to put code needed only for hard faults in a different color}
% Guy: could not figure out how to do this easily, and some code is hard to separate
}
\label{WS-deque-fig}
\end{figure}

